ETL for the integration of remote sensing data

Modern in-orbit satellites and other available remote sensing tools have generated a huge availability of public data waiting to be exploited in different formats hosted on different servers. In this context, ETL formalism becomes relevant for the integration and analysis of the combined information from all these sources. Throughout this work, we present the theoretical and practical foundations to build a modular analysis infrastructure that allows the creation of ETLs to download, transform and integrate data coming from different instruments in different formats. Part of this work is already implemented in a Python library which is intended to be integrated into already available workflow management tools based on acyclic-directed graphs which also have different adapters to impact the combined data in different warehouses.

==> macros.tex <==
\input{macros}

\newcommand{\citeme}{{\color{red}{¡¡CITEME: ##1 !!}}}
\newcommand{\pau}[1]{{\color{violet} #1}}
